Intrinsically-Motivated Reinforcement Learning: A Brief Introduction

Reinforcement learning (RL) is one of the three basic paradigms of machine learning. It has demonstrated impressive performance in many complex tasks like Go and StarCraft, which is increasingly involved in smart manufacturing and autonomous driving. However, RL consistently suffers from the exploration-exploitation dilemma. In this paper, we investigated the problem of improving exploration in RL and introduced the intrinsically-motivated RL. In sharp contrast to the classic exploration strategies, intrinsically-motivated RL utilizes the intrinsic learning motivation to provide sustainable exploration incentives. We carefully classified the existing intrinsic reward methods and analyzed their practical drawbacks. Moreover, we proposed a new intrinsic reward method via R\'enyi state entropy maximization, which overcomes the drawbacks of the preceding methods and provides powerful exploration incentives. Finally, extensive simulation demonstrated that the proposed module achieve superior performance with higher efficiency and robustness.

==> figures/plotbatrj.tex <==
% \documentclass{standalone}
% \usepackage{tikz}
% \usepackage{pgfplots}

% \begin{document}

\begin{tikzpicture}
\begin{axis}[
    axis equal=true,
    small,
    width=10cm,
    height=6cm,
    title={Trajectories: \textit{Dataset Room}},
    xlabel={x [m]},
    ylabel={y [m]},
    grid=major,
    grid style={dotted},
    % xmin=0,xmax=85,
    % grid=major,
    legend style={
      at={(0.6,0.75)},
      font=\footnotesize,
    },
]
\addplot [black,thick] table {figures/ba-r4-007.traj-odoerrTruetrj.dat};
\addplot [red,densely dashed] table {figures/ba-r4-007.traj-odoerrOdometrytrj.dat};
\addplot [blue,thin] table {figures/ba-r4-007.traj-odoerrORB-SLAMtrj.dat};
\addplot [green!50!black!80,thick] table {figures/ba-r4-007.traj-odoerrOurstrj.dat};
\legend{Truth,Odometry,ORB-SLAM, Ours},
\end{axis}
\end{tikzpicture}
% \end{document}


==> figures/pose_motivation.tex <==
\begin{tikzpicture}[>=latex,scale=1.0,
  ]

  \def\cameraicon#1#2{
    \begin{scope}[shift={#1}, rotate=#2]
      \draw[thick,fill=white] (-0.3,-0.2) -- (0.3,-0.2) -- (0.3,0.2) -- (0.2,0.2) --
      (0.16,0.24) -- (-0.16,0.24)--(-0.2,0.2)--(-0.3,0.2)--cycle;
      \draw[thick,fill=white] (0,0.02) circle [radius=0.15];
    \end{scope}
  }
  % \draw[gray!50,step=0.5] (0,0) grid (12,6);
  \foreach \x in {0.5,4.5,8.5}
  {
    \draw[thick] (\x,2) rectangle (\x+2.5,3);
    \draw[thick,fill=white] (\x+0.5,2) circle [radius=0.25];
    \draw[thick,fill=white] (\x+2,2) circle [radius=0.25];
    \draw[blue!50] (\x+1.5,5) node {\Large $\bigstar$};
    \draw[blue!50] (\x+0.8,5) node {\small XYZ};
    \cameraicon{(\x+1.25,3)}{0}
    \draw[blue!50,thick,->] (\x+1.25,3) -- (\x+1.5,4.9);
  }
  \foreach \x in {1,2,3,4,5,6,7,8}
  {
    \draw (4.5+\x*0.30,1.75) -- +(-0.25,-0.3);
    \draw[xshift=4cm,yshift=-0.25cm] (4.5+\x*0.30,1.75) -- +(-0.25,-0.3);
  }
  \draw[] (1.75,2.4) node {\small SE(3)};
  \draw[] (5.75,2.4) node {\small SE(2)};
  \draw[] (9.75,2.4) node {\small SE(3)};
  \draw[yshift=0.25cm] (7,1.2) node[fill=white] {\small SE(2)};
  \draw[xshift=4cm] (7,1.2) node[fill=white] {\small SE(2)};
  \draw[thick] (4.5,1.75) -- (7,1.75);
  \draw[thick,xshift=4cm,yshift=-0.25cm] (4.5,1.75) -- (7,1.75);
  \draw[very thick] (9.7,1.5) -- (10,1.65) -- (9.5,1.65) -- (10,1.85) -- (9.5,1.85) --(9.9,2);

  \draw (0.5,0.8) node[below right,align=left] {\small Unconstrained\\ SE(3) poses};
  \draw[xshift=4cm] (0.5,0.8) node[below right,align=left] {\small Deterministic\\ SE(2)-constraints};
  \draw[xshift=8cm] (0.5,0.8) node[below right,align=left] {\small Stochastic\\ SE(2)-constraints\\ on SE(3) poses};

\end{tikzpicture}


==> sections/abstract.tex <==
Reinforcement learning (RL) is one of the three basic paradigms of machine learning. It has demonstrated impressive performance in many complex tasks like Go and StarCraft, which is increasingly involved in smart manufacturing and autonomous driving. However, RL consistently suffers from the exploration-exploitation dilemma. In this paper, we investigated the problem of improving exploration in RL and introduced the intrinsically-motivated RL. In sharp contrast to the classic exploration strategies, intrinsically-motivated RL utilizes the intrinsic learning motivation to provide sustainable exploration incentives. We carefully classified the existing intrinsic reward methods and analyzed their practical drawbacks. Moreover, we proposed a new intrinsic reward method via R\'enyi state entropy maximization, which overcomes the drawbacks of the preceding methods and provides powerful exploration incentives. Finally, extensive simulation demonstrated that the proposed module achieve superior performance with higher efficiency and robustness.




==> sections/dedication.tex <==
Dedicated to those who risked their life fighting against \mbox{COVID-19}.


==> sections/proof.tex <==
\chapter{Proof of Propositions} 


\section{Network Architectures}


\section{Hyper-parameters Setting}

\chapterend


==> sections/publications.tex <==
\chapter{Publication List}

\begin{itemize}
	\item M. Yuan, Q. Cao, M. -O. Pun and Y. Chen, "Multi-Agent Reinforcement Learning-Based Fairness-Aware Scheduling for Bursty Traffic," 2021 IEEE Global Communications Conference (GLOBECOM), 2021, pp. 1-6, doi: 10.1109/GLOBECOM46510.2021.9685661.
	\item Y. Xu, M. Yuan and M. -O. Pun, "Transformer Empowered CSI Feedback for Massive MIMO Systems," 2021 30th Wireless and Optical Communications Conference (WOCC), 2021, pp. 157-161, doi: 10.1109/WOCC53213.2021.9602863.
	\item M. Yuan and M. -O. Pun, "Exploring Beyond-Demonstrator via Meta Learning-Based Reward Extrapolation," \textbf{submitted to} 2022 IEEE/RSJ International Conference on Intelligent Robots and Systems (IROS).
	\item M. Yuan, M. -O. Pun and D. Wang, "Rényi State Entropy for Accelerating Exploration in Reinforcement Learning," \textbf{submitted to} IEEE Transactions on Artificial Intelligence (TAI).
\end{itemize}

\chapterend



==> sections/symbols-and-acronyms.tex <==
\chapter*{Symbols and Acronyms}
\addcontentsline{toc}{chapter}{Symbols and Acronyms}

In general, we denote a scalar by an italic lower case letter,
a vector by a roman lower case bold letter,
and a matrix by a roman upper case bold letter respectively, e.g.,
$a \in \bbR$, $\mathbf{v} \in \bbR^n$ and $\mathbf{M} \in \bbR^{p \times q}$, with any exceptions to be mentioned in the context case by case.

Specifically, the components of any vector ${\bf v} \in \bbR^2$ or ${\bf v}\in \bbR^3$ are written as $[v_x\,v_y]^T$ or $[v_x\,v_y\,v_z]^T$.

An identity matrix is written as $\bI$. Specifically, an $n\times n$ identity matrix is written as $\bI_n$.
A zero matrix or vector is written as ${\bf 0}$. Specifically, an $m\times n$ zero matrix is written as ${\bf 0}_{m\times n}$.

$\check{(\cdot)}$ denotes the prior of any quantity, while $\hat{(\cdot)}$ denotes the posterior.

Specialized symbols and major acronyms are defined as follows:

\newpage

\noindent
$\mathbbm{1}$ \hfill the indicator function \\
$\ominus$ \hfill the Euclidean distance \\
$\oplus$ \hfill the summation operation \\
$H$ \hfill the Shannon entropy \\
$H_{\alpha}$ \hfill the \Ry entropy \\
$\bm{s}$ \hfill a state \\
$\bm{a}$ \hfill an action \\
$\pi$ \hfill a policy \\
$p(\cdot)$ \hfill the probability density function \\
$r(\cdot)$ \hfill the reward function \\
$\rho(\cdot)$ \hfill the initial state distribution \\
$\gamma$ \hfill a discount factor \\
$D_{\rm KL}$ \hfill the Kullback–Leibler divergence \\
$D_{\rm M}$ \hfill the Manhattan distance \\
$\mathcal{M}$ \hfill a Markov decision process \\
$\mathcal{S}$ \hfill a state space \\
$\mathcal{A}$ \hfill an action space \\
$\mathcal{T}$ \hfill a transition probability distribution \\
$\mathcal{N}$ \hfill a noise process \\
$\mathbb{E}$ \hfill the expectation \\
$\tr(\cdot)$ \hfill trace of a matrix \\
$\det(\cdot)$ \hfill determinant of a matrix \\



\newpage
\noindent
CCP       \hfill coupon collector's problem					  \\
GIRM 	  \hfill generative intrinsic reward module			  \\
ICM 	  \hfill intrinsic curiosity module					  \\
RL        \hfill reinforcement learning                       \\
MDP 	  \hfill Markov decision process                      \\
MSE 	  \hfill mean squared error                           \\
NGU       \hfill never give up								  \\
OUP       \hfill Ornstein-Uhlenbeck process					  \\
PBRS      \hfill potential-based reward shaping               \\
PG        \hfill prediction gain							  \\
PPO 	  \hfill proximal policy optimization				  \\
RISE      \hfill \Ry state entropy                            \\
RE3       \hfill random encoders for efficient exploration    \\
RIDE      \hfill reward impact-driven exploration 			  \\
RND 	  \hfill random network distillation 				  \\
TS 		  \hfill Thompson sampling 						 	  \\
UCB       \hfill upper confidence bound 					  \\
VAE       \hfill variational auto-encoder					  \\
VPG 	  \hfill vanilla policy gradient 					  \\

